CKH: Causal Knowledge Hierarchy for Estimating Structural Causal Models from Data and Priors

Structural causal models (SCMs) provide a principled approach to identifying causation from observational and experimental data in disciplines ranging from economics to medicine. However, SCMs, which is typically represented as graphical models, cannot rely only on data, rather require support of domain knowledge. A key challenge in this context is the absence of a methodological framework for encoding priors (background knowledge) into causal models in a systematic manner. We propose an abstraction called causal knowledge hierarchy (CKH) for encoding priors into causal models. Our approach is based on the foundation of "levels of evidence" in medicine, with a focus on confidence in causal information. Using CKH, we present a methodological framework for encoding causal priors from various information sources and combining them to derive an SCM. We evaluate our approach on a simulated dataset and demonstrate overall performance compared to the ground truth causal model with sensitivity analysis.

==> sections/checklist.tex <==
\section{Checklist}
\begin{enumerate}
    \item Address NIPS reviews: https://docs.google.com/document/d/1zvrrPvFdY-FMUdQ53g0KuY3NYNT27dvdGmwLuAfpTaU/edit
    \item Reproducibility checklist in new submission: https://docs.google.com/document/d/1XUt-9opit6-NZ8gTWr39VwQmYjypbfL10rHwu5lnFss/edit?usp=sharing
    \item (theory) Theoretical robustness 
    \item (theory) Completeness proof 
    \item (simulation) Real-world data driven model generation / known causal model generation 
    \item (validation) True positive rate (TPR), False discovery rate (FDR), and Matthew’s correlation coefficient (MCC)  
    \item add new table
    \item reformat to aaai
\end{enumerate}
